Function Norms and Regularization in Deep Networks

Deep neural networks (DNNs) have become increasingly important due to their excellent empirical performance on a wide range of problems. However, regularization is generally achieved by indirect means, largely due to the complex set of functions defined by a network and the difficulty in measuring function complexity. There exists no method in the literature for additive regularization based on a norm of the function, as is classically considered in statistical learning theory. In this work, we propose sampling-based approximations to weighted function norms as regularizers for deep neural networks. We provide, to the best of our knowledge, the first proof in the literature of the NP-hardness of computing function norms of DNNs, motivating the necessity of an approximate approach. We then derive a generalization bound for functions trained with weighted norms and prove that a natural stochastic optimization strategy minimizes the bound. Finally, we empirically validate the improved performance of the proposed regularization strategies for both convex function sets as well as DNNs on real-world classification and image segmentation tasks demonstrating improved performance over weight decay, dropout, and batch normalization. Source code will be released at the time of publication.

==> architectures.tex <==
\begin{table}[t!]
\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \hline
    Block    & conv kernel     & \# filters     & dilation  & pool kernel   & pool stride   & batch norm.\\\hline
	1         & 7$\times$7      & 64           & 1				& 3$\times 3$   & 2      		& yes     \\\hline
	2     	 & 5$\times$5     & 128            & 1  			& 3$\times 3$   & 2      		   & yes     \\\hline
	3         & 3$\times$3      & 256          & 2				& 3$\times 3$   & 1       	   & yes    \\\hline
	4         & 3$\times$3      & 512          & 2  			& 3$\times 3$   & 1       	   & yes    \\\hline
	5         & 3$\times$3      & 512          & 2				& 3$\times 3$   & 1       	   & yes    \\\hline
	6         & 4$\times$4      & 1024         & 4				& no pooling    &        		& yes    \\\hline
	7         & 1$\times$1      & 39           & 1				& no pooling    &        		& no     \\\hline
    \end{tabular}
    }
    \caption{Layers used for the brain image segmentation.}
    \label{tab:architecture}
\end{table}
